The Outcome of the 2022 Landslide4Sense Competition: Advanced Landslide Detection from Multi-Source Satellite Imagery

The scientific outcomes of the 2022 Landslide4Sense (L4S) competition organized by the Institute of Advanced Research in Artificial Intelligence (IARAI) are presented here. The objective of the competition is to automatically detect landslides based on large-scale multiple sources of satellite imagery collected globally. The 2022 L4S aims to foster interdisciplinary research on recent developments in deep learning (DL) models for the semantic segmentation task using satellite imagery. In the past few years, DL-based models have achieved performance that meets expectations on image interpretation, due to the development of convolutional neural networks (CNNs). The main objective of this article is to present the details and the best-performing algorithms featured in this competition. The winning solutions are elaborated with state-of-the-art models like the Swin Transformer, SegFormer, and U-Net. Advanced machine learning techniques and strategies such as hard example mining, self-training, and mix-up data augmentation are also considered. Moreover, we describe the L4S benchmark data set in order to facilitate further comparisons, and report the results of the accuracy assessment online. The data is accessible on \textit{Future Development Leaderboard} for future evaluation at \url{https://www.iarai.ac.at/landslide4sense/challenge/}, and researchers are invited to submit more prediction results, evaluate the accuracy of their methods, compare them with those of other users, and, ideally, improve the landslide detection results reported in this article.

==> table_top-teams.tex <==
\begin{table*}[ht]
\caption{Top ranked teams and their approaches.}
\label{tab:ranking}
\centering
\scriptsize
\begin{tabular}{c c c c c c c c c c c}
\toprule
\multirow{2}{*}{Rank} & \multirow{2}{*}{Team} & \multirow{2}{*}{mIoU} & \multicolumn{2}{c}{Data} & \multicolumn{6}{c}{Approach} \\
\cmidrule(l{2pt}r{2pt}){4-5}
\cmidrule(l{2pt}r{2pt}){6-11}
  &  &  & L8 & Other & Ensemble & 
\begin{tabular}{c}
Refine \\
LR labels
\end{tabular}
  & 
\begin{tabular}{c}
Pseudo \\
labels
\end{tabular}  
  & Multi-task &
\begin{tabular}{c}
Specific \\
class
\end{tabular}
& 
\begin{tabular}{c}
Filtering, \\
thresholding
\end{tabular}  
  \\
\midrule
 1 & \textit{AsheLee}    & 0.6772 & $\checkmark$ &  & $\checkmark$ & $\checkmark$ & $\checkmark$ &$\checkmark$ &  & $\checkmark$ \\
 2 & \textit{tulilin}    & 0.6657 &$\checkmark$  & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ &  & & $\checkmark$ \\
 3 & \textit{baoqianyue} & 0.6445 &  & & $\checkmark$ &  & $\checkmark$  &              & $\checkmark$ & \\
 4 & \textit{EVER}       & 0.6435 & $\checkmark$ &  &              &  &  $\checkmark$  & $\checkmark$ &  & $\checkmark$  \\
\bottomrule
\end{tabular}
\end{table*}
